The impact of magnetic fields on cosmological galaxy mergers -- II. Modified angular momentum transport and feedback

The role of magnetic fields in galaxy evolution is still an unsolved question in astrophysics. We have previously shown that magnetic fields play a crucial role in major mergers between disc galaxies; in hydrodynamic simulations of such mergers, the Auriga model produces compact remnants with a distinctive bar and ring morphology. In contrast, in magnetohydrodynamic (MHD) simulations, remnants form radially-extended discs with prominent spiral arm structure. In this paper, we analyse a series of cosmological "zoom-in" simulations of major mergers and identify exactly \textit{how} magnetic fields are able to alter the outcome of the merger. We find that magnetic fields modify the transport of angular momentum, systematically hastening the merger progress. The impact of this altered transport depends on the orientation of the field, with a predominantly non-azimuthal (azimuthal) orientation increasing the central baryonic concentration (providing support against collapse). Both effects act to suppress an otherwise existent bar-instability, which in turn leads to a fundamentally different morphology and manifestation of feedback. We note, in particular, that stellar feedback is substantially less influential in MHD simulations, which allows for the later accretion of higher angular momentum gas and the subsequent rapid radial growth of the remnant disc. A corollary of the increased baryonic concentration in MHD simulations is that black holes are able to grow twice as large, although this turns out to have little impact on the remnant's development. Our results show that galaxy evolution cannot be modelled correctly without including magnetic fields.

==> Makefile <==
# Makefile to produce the article.
PDFLATEX  =  TEXINPUTS=.//: BSTINPUTS=.//: pdflatex
LATEX  =  TEXINPUTS=.//: BSTINPUTS=.//: latex
DVIPS  =  dvips
FIGURES = 

.PRECIOUS: $(FIGURES)

default: main.pdf

%.pdf :  $(FIGURES) %.tex
	$(PDFLATEX) $*.tex
	TEXINPUTS=:.// BSTINPUTS=:.// bibtex $*
	$(PDFLATEX) $*.tex
	$(PDFLATEX) $*.tex
	$(PDFLATEX) $*.tex
	make clean

%.ps :  $(FIGURES) %.tex
	$(LATEX) $*.tex
	TEXINPUTS=:.// BSTINPUTS=:.// bibtex $*
	$(LATEX) $*.tex
	$(LATEX) $*.tex
	$(LATEX) $*.tex
	$(DVIPS) -o $*.ps $*.dvi
	ps2pdf $*.ps
	make clean

figures/%.eps: figures/%_raw.eps figures/%.tex
	(cd figures; latex $*.tex; \
	dvips -E -o $*.eps $*.dvi; \
	perl -ane '{ s/%%BoundingBox: [-0-9]+/%%BoundingBox: 135/g; print}' $*.eps > tmp.eps; \
	mv tmp.eps $*.eps; \
	rm -f *.dvi *.log *.aux)

clean:
	rm -f *.log *.toc *.aux *.dvi *.bak *.blg *.obj *.out

realclean:
	rm -f *.log *.toc *.aux *.dvi *.obj *.bak *.bbl *.blg *.brf \
              *.pdf *.ps */*.ps *~ */*~ *.bak */*.bak 









